Zoom In and Out: A Mixed-scale Triplet Network for Camouflaged Object Detection

The recently proposed camouflaged object detection (COD) attempts to segment objects that are visually blended into their surroundings, which is extremely complex and difficult in real-world scenarios. Apart from high intrinsic similarity between the camouflaged objects and their background, the objects are usually diverse in scale, fuzzy in appearance, and even severely occluded. To deal with these problems, we propose a mixed-scale triplet network, \textbf{ZoomNet}, which mimics the behavior of humans when observing vague images, i.e., zooming in and out. Specifically, our ZoomNet employs the zoom strategy to learn the discriminative mixed-scale semantics by the designed scale integration unit and hierarchical mixed-scale unit, which fully explores imperceptible clues between the candidate objects and background surroundings. Moreover, considering the uncertainty and ambiguity derived from indistinguishable textures, we construct a simple yet effective regularization constraint, uncertainty-aware loss, to promote the model to accurately produce predictions with higher confidence in candidate regions. Without bells and whistles, our proposed highly task-friendly model consistently surpasses the existing 23 state-of-the-art methods on four public datasets. Besides, the superior performance over the recent cutting-edge models on the SOD task also verifies the effectiveness and generality of our model. The code will be available at \url{https://github.com/lartpang/ZoomNet}.

==> tables/detail_totalsod.tex <==
\begin{tabular}{cc|ccccccccccc}
 \toprule[2pt]
 \rowcolor{tabtitle}
                                                       &                                 & \textbf{DGRL}    & \textbf{PAGRN}    & \textbf{PiCANet}                 & \textbf{RAS}                     & \textbf{AFNet}                   & \textbf{BASNet}                  & \textbf{CPD}                     & \textbf{PoolNet}                & \textbf{EGNet}                   & \textbf{HRS}                     & \textbf{ICNet}                   \\ \rowcolor{tabtitle}
 \multicolumn{2}{c|}{\multirow{-2}{*}{\textbf{MODEL}}} & \cite{DGRL}                     & \cite{PAGRN}     & \cite{PiCANet}    & \cite{RAS}                       & \cite{AFNetRGB}                  & \cite{BASNet}                    & \cite{CPD}                       & \cite{PoolNet}                   & \cite{EGNet}                    & \cite{HRS}                       & \cite{ICNet}                                                        \\ \midrule[1pt]
                                                       & S$_{m}$ $\uparrow$              & 0.810            & 0.775             & 0.832                            & 0.814                            & 0.826                            & 0.836                            & 0.825                            & 0.831                           & {\color{mygreen} \textbf{0.841}} & 0.772                            & 0.837                            \\
                                                       & F$^{\omega}_{\beta}$ $\uparrow$ & 0.697            & 0.622             & 0.695                            & 0.695                            & 0.717                            & {\color{myblue} \textbf{0.751}}  & 0.719                            & 0.725                           & 0.738                            & 0.645                            & 0.730                            \\
                                                       & MAE $\downarrow$                & 0.063            & 0.071             & 0.065                            & 0.062                            & 0.057                            & 0.056                            & 0.056                            & 0.054                           & {\color{myblue} \textbf{0.053}}  & 0.066                            & 0.061                            \\
                                                       & F$^{adp}_{\beta}$ $\uparrow$    & 0.709            & 0.711             & 0.717                            & 0.713                            & 0.739                            & 0.756                            & 0.747                            & 0.752                           & 0.756                            & 0.708                            & 0.739                            \\
                                                       & F$^{avg}_{\beta}$ $\uparrow$    & 0.726            & 0.675             & 0.729                            & 0.731                            & 0.742                            & 0.767                            & 0.742                            & 0.747                           & 0.760                            & 0.690                            & 0.760                            \\
                                                       & E$^{adp}_{m}$ $\uparrow$        & 0.850            & 0.843             & 0.848                            & 0.849                            & 0.859                            & 0.869                            & 0.873                            & 0.874                           & 0.874                            & 0.842                            & 0.859                            \\
 \multirow{-7}{*}{\rotatebox{90}{\textbf{DUT-OMRON}}}  & E$^{avg}_{m}$ $\uparrow$        & 0.845            & 0.772             & 0.836                            & 0.843                            & 0.846                            & {\color{myblue} \textbf{0.865}}  & 0.847                            & 0.848                           & 0.857                            & 0.791                            & {\color{mygreen} \textbf{0.867}} \\ \hline
                                                       & S$_{m}$ $\uparrow$              & 0.842            & 0.839             & 0.869                            & 0.839                            & 0.867                            & 0.866                            & 0.869                            & 0.887                           & 0.887                            & 0.829                            & 0.865                            \\
                                                       & F$^{\omega}_{\beta}$ $\uparrow$ & 0.774            & 0.724             & 0.755                            & 0.740                            & 0.785                            & 0.803                            & 0.795                            & 0.817                           & 0.816                            & 0.746                            & 0.762                            \\
                                                       & MAE $\downarrow$                & 0.050            & 0.055             & 0.051                            & 0.059                            & 0.046                            & 0.048                            & 0.043                            & 0.037                           & 0.039                            & 0.051                            & 0.048                            \\
                                                       & F$^{adp}_{\beta}$ $\uparrow$    & 0.794            & 0.784             & 0.759                            & 0.751                            & 0.793                            & 0.791                            & 0.805                            & 0.819                           & 0.815                            & 0.793                            & 0.767                            \\
                                                       & F$^{avg}_{\beta}$ $\uparrow$    & 0.797            & 0.778             & 0.791                            & 0.779                            & 0.812                            & 0.823                            & 0.821                            & 0.840                           & 0.839                            & 0.791                            & 0.804                            \\
                                                       & E$^{adp}_{m}$ $\uparrow$        & 0.899            & 0.883             & 0.873                            & 0.864                            & 0.895                            & 0.884                            & 0.904                            & 0.912                           & 0.907                            & 0.889                            & 0.880                            \\
 \multirow{-7}{*}{\rotatebox{90}{\textbf{DUTS-TE}}}    & E$^{avg}_{m}$ $\uparrow$        & 0.894            & 0.842             & 0.878                            & 0.871                            & 0.893                            & 0.895                            & 0.898                            & 0.910                           & 0.907                            & 0.861                            & 0.892                            \\ \hline
                                                       & S$_{m}$ $\uparrow$              & 0.906            & 0.889             & 0.917                            & 0.893                            & 0.913                            & 0.916                            & 0.918                            & {\color{myblue} \textbf{0.926}} & 0.925                            & 0.883                            & 0.918                            \\
                                                       & F$^{\omega}_{\beta}$ $\uparrow$ & 0.883            & 0.834             & 0.867                            & 0.857                            & 0.886                            & 0.904                            & 0.898                            & 0.904                           & 0.903                            & 0.859                            & 0.881                            \\
                                                       & MAE $\downarrow$                & 0.043            & 0.061             & 0.046                            & 0.056                            & 0.042                            & 0.037                            & 0.037                            & 0.035                           & 0.037                            & 0.054                            & 0.041                            \\
                                                       & F$^{adp}_{\beta}$ $\uparrow$    & 0.903            & 0.894             & 0.886                            & 0.889                            & 0.908                            & 0.880                            & 0.917                            & 0.919                           & 0.920                            & 0.902                            & 0.880                            \\
                                                       & F$^{avg}_{\beta}$ $\uparrow$    & 0.900            & 0.877             & 0.890                            & 0.887                            & 0.905                            & 0.917                            & 0.913                            & 0.918                           & 0.918                            & 0.894                            & 0.904                            \\
                                                       & E$^{adp}_{m}$ $\uparrow$        & 0.943            & 0.917             & 0.927                            & 0.922                            & 0.941                            & 0.921                            & 0.949                            & 0.948                           & 0.947                            & 0.923                            & 0.924                            \\
 \multirow{-7}{*}{\rotatebox{90}{\textbf{ECSSD}}}      & E$^{avg}_{m}$ $\uparrow$        & 0.938            & 0.893             & 0.925                            & 0.914                            & 0.935                            & 0.943                            & 0.942                            & 0.945                           & 0.943                            & 0.911                            & 0.937                            \\ \hline
                                                       & S$_{m}$ $\uparrow$              & 0.897            & 0.887             & 0.904                            & 0.887                            & 0.905                            & 0.909                            & 0.905                            & {\color{myblue} \textbf{0.919}} & 0.918                            & 0.882                            & 0.907                            \\
                                                       & F$^{\omega}_{\beta}$ $\uparrow$ & 0.865            & 0.820             & 0.840                            & 0.843                            & 0.869                            & 0.889                            & 0.875                            & 0.888                           & 0.887                            & 0.851                            & 0.856                            \\
                                                       & MAE $\downarrow$                & 0.037            & 0.048             & 0.043                            & 0.045                            & 0.036                            & 0.032                            & 0.034                            & 0.030                           & 0.031                            & 0.042                            & 0.038                            \\
                                                       & F$^{adp}_{\beta}$ $\uparrow$    & 0.882            & 0.886             & 0.870                            & 0.871                            & 0.888                            & 0.895                            & 0.891                            & 0.903                           & 0.901                            & 0.891                            & 0.878                            \\
                                                       & F$^{avg}_{\beta}$ $\uparrow$    & 0.884            & 0.864             & 0.866                            & 0.875                            & 0.888                            & 0.902                            & 0.892                            & 0.903                           & 0.902                            & 0.883                            & 0.883                            \\
                                                       & E$^{adp}_{m}$ $\uparrow$        & 0.946            & 0.939             & 0.940                            & 0.931                            & 0.947                            & 0.946                            & 0.950                            & {\color{myblue} \textbf{0.959}} & 0.956                            & 0.937                            & 0.942                            \\
 \multirow{-7}{*}{\rotatebox{90}{\textbf{HKU-IS}}}     & E$^{avg}_{m}$ $\uparrow$        & 0.939            & 0.898             & 0.916                            & 0.920                            & 0.934                            & 0.943                            & 0.938                            & 0.945                           & 0.944                            & 0.918                            & 0.933                            \\ \hline
                                                       & S$_{m}$ $\uparrow$              & 0.837            & 0.814             & 0.852                            & 0.793                            & 0.850                            & 0.834                            & 0.844                            & {\color{myblue} \textbf{0.864}} & 0.850                            & 0.799                            & 0.849                            \\
                                                       & F$^{\omega}_{\beta}$ $\uparrow$ & 0.790            & 0.734             & 0.779                            & 0.735                            & 0.804                            & 0.797                            & 0.800                            & 0.819                           & 0.804                            & 0.744                            & 0.789                            \\
                                                       & MAE $\downarrow$                & 0.076            & 0.095             & 0.078                            & 0.106                            & 0.071                            & 0.079                            & 0.074                            & 0.067                           & 0.076                            & 0.091                            & 0.072                            \\
                                                       & F$^{adp}_{\beta}$ $\uparrow$    & 0.812            & 0.805             & 0.802                            & 0.785                            & 0.828                            & 0.777                            & 0.829                            & 0.838                           & 0.829                            & 0.806                            & 0.785                            \\
                                                       & F$^{avg}_{\beta}$ $\uparrow$    & 0.821            & 0.790             & 0.812                            & 0.790                            & 0.832                            & 0.824                            & 0.827                            & 0.846                           & 0.833                            & 0.792                            & 0.824                            \\
                                                       & E$^{adp}_{m}$ $\uparrow$        & 0.879            & 0.851             & 0.860                            & 0.834                            & 0.887                            & 0.850                            & 0.885                            & 0.888                           & 0.877                            & 0.847                            & 0.859                            \\
 \multirow{-7}{*}{\rotatebox{90}{\textbf{PASCAL-S}}}   & E$^{avg}_{m}$ $\uparrow$        & 0.881            & 0.826             & 0.868                            & 0.829                            & 0.884                            & 0.876                            & 0.879                            & 0.894                           & 0.880                            & 0.829                            & 0.884                            \\
 \bottomrule[1pt]
 \rowcolor{tabtitle}
                                                       &                                 & \textbf{MLMSNet} & \textbf{PAGE-Net} & \textbf{SCRN}                    & \textbf{F3Net}                   & \textbf{GCPANet}                 & \textbf{LDF}                     & \textbf{DFI}                     & \textbf{GateNet}                & \textbf{ITSD}                    & \textbf{MINet}                   & \textbf{Ours}                    \\ \rowcolor{tabtitle}
 \multicolumn{2}{c|}{\multirow{-2}{*}{\textbf{MODEL}}} & \cite{MLMSNet}                  & \cite{PAGE-Net}  & \cite{SCRN}       & \cite{F3Net}                     & \cite{GCPANet}                   & \cite{LDF}                       & \cite{DFI}                       & \cite{GateNet}                   & \cite{ITSD}                     & \cite{MINet}                     &                                                                     \\ \midrule[1pt]
                                                       & S$_{m}$ $\uparrow$              & 0.809            & 0.824             & 0.837                            & 0.838                            & 0.839                            & 0.839                            & {\color{myblue} \textbf{0.840}}  & 0.838                           & {\color{myblue} \textbf{0.840}}  & 0.833                            & {\color{reda} \textbf{0.844}}    \\
                                                       & F$^{\omega}_{\beta}$ $\uparrow$ & 0.681            & 0.722             & 0.720                            & 0.747                            & 0.734                            & {\color{mygreen} \textbf{0.752}} & 0.738                            & 0.729                           & 0.750                            & 0.738                            & {\color{reda} \textbf{0.761}}    \\
                                                       & MAE $\downarrow$                & 0.064            & 0.062             & 0.056                            & {\color{myblue} \textbf{0.053}}  & 0.056                            & {\color{mygreen} \textbf{0.052}} & 0.055                            & 0.055                           & 0.061                            & 0.056                            & {\color{reda} \textbf{0.049}}    \\
                                                       & F$^{adp}_{\beta}$ $\uparrow$    & 0.692            & 0.736             & 0.746                            & {\color{myblue} \textbf{0.766}}  & 0.748                            & {\color{mygreen} \textbf{0.773}} & 0.752                            & 0.746                           & 0.756                            & 0.755                            & {\color{reda} \textbf{0.780}}    \\
                                                       & F$^{avg}_{\beta}$ $\uparrow$    & 0.710            & 0.743             & 0.749                            & 0.766                            & 0.756                            & {\color{mygreen} \textbf{0.770}} & 0.762                            & 0.757                           & {\color{myblue} \textbf{0.768}}  & 0.757                            & {\color{reda} \textbf{0.776}}    \\
                                                       & E$^{adp}_{m}$ $\uparrow$        & 0.839            & 0.860             & 0.869                            & {\color{myblue} \textbf{0.876}}  & 0.869                            & {\color{reda} \textbf{0.881}}    & 0.870                            & 0.868                           & 0.867                            & 0.873                            & {\color{mygreen} \textbf{0.879}} \\
 \multirow{-7}{*}{\rotatebox{90}{\textbf{DUT-OMRON}}}  & E$^{avg}_{m}$ $\uparrow$        & 0.831            & 0.849             & 0.848                            & 0.864                            & 0.853                            & {\color{myblue} \textbf{0.865}}  & 0.862                            & 0.855                           & {\color{myblue} \textbf{0.865}}  & 0.860                            & {\color{reda} \textbf{0.868}}    \\ \hline
                                                       & S$_{m}$ $\uparrow$              & 0.862            & 0.854             & 0.885                            & 0.888                            & {\color{myblue} \textbf{0.891}}  & {\color{mygreen} \textbf{0.892}} & 0.887                            & 0.885                           & 0.885                            & 0.884                            & {\color{reda} \textbf{0.905}}    \\
                                                       & F$^{\omega}_{\beta}$ $\uparrow$ & 0.761            & 0.769             & 0.803                            & {\color{myblue} \textbf{0.835}}  & 0.821                            & {\color{mygreen} \textbf{0.845}} & 0.817                            & 0.809                           & 0.824                            & 0.825                            & {\color{reda} \textbf{0.866}}    \\
                                                       & MAE $\downarrow$                & 0.049            & 0.052             & 0.040                            & {\color{myblue} \textbf{0.035}}  & 0.038                            & {\color{mygreen} \textbf{0.034}} & 0.039                            & 0.040                           & 0.041                            & 0.037                            & {\color{reda} \textbf{0.029}}    \\
                                                       & F$^{adp}_{\beta}$ $\uparrow$    & 0.745            & 0.777             & 0.809                            & {\color{myblue} \textbf{0.840}}  & 0.817                            & {\color{mygreen} \textbf{0.855}} & 0.814                            & 0.807                           & 0.804                            & 0.828                            & {\color{reda} \textbf{0.867}}    \\
                                                       & F$^{avg}_{\beta}$ $\uparrow$    & 0.792            & 0.793             & 0.833                            & {\color{myblue} \textbf{0.852}}  & 0.841                            & {\color{mygreen} \textbf{0.861}} & 0.840                            & 0.837                           & 0.840                            & 0.844                            & {\color{reda} \textbf{0.878}}    \\
                                                       & E$^{adp}_{m}$ $\uparrow$        & 0.863            & 0.886             & 0.901                            & {\color{myblue} \textbf{0.918}}  & 0.913                            & {\color{mygreen} \textbf{0.929}} & 0.908                            & 0.903                           & 0.898                            & 0.917                            & {\color{reda} \textbf{0.939}}    \\
 \multirow{-7}{*}{\rotatebox{90}{\textbf{DUTS-TE}}}    & E$^{avg}_{m}$ $\uparrow$        & 0.883            & 0.883             & 0.900                            & {\color{myblue} \textbf{0.920}}  & 0.911                            & {\color{mygreen} \textbf{0.925}} & 0.912                            & 0.906                           & 0.913                            & 0.917                            & {\color{reda} \textbf{0.938}}    \\ \hline
                                                       & S$_{m}$ $\uparrow$              & 0.911            & 0.912             & {\color{mygreen} \textbf{0.927}} & 0.924                            & {\color{mygreen} \textbf{0.927}} & 0.924                            & {\color{mygreen} \textbf{0.927}} & 0.920                           & 0.925                            & 0.925                            & {\color{reda} \textbf{0.930}}    \\
                                                       & F$^{\omega}_{\beta}$ $\uparrow$ & 0.871            & 0.886             & 0.900                            & {\color{myblue} \textbf{0.912}}  & 0.903                            & {\color{mygreen} \textbf{0.915}} & 0.906                            & 0.894                           & 0.910                            & 0.911                            & {\color{reda} \textbf{0.922}}    \\
                                                       & MAE $\downarrow$                & 0.045            & 0.042             & 0.037                            & {\color{mygreen} \textbf{0.033}} & 0.035                            & {\color{myblue} \textbf{0.034}}  & 0.035                            & 0.040                           & {\color{myblue} \textbf{0.034}}  & {\color{mygreen} \textbf{0.033}} & {\color{reda} \textbf{0.030}}    \\
                                                       & F$^{adp}_{\beta}$ $\uparrow$    & 0.868            & 0.906             & 0.918                            & {\color{myblue} \textbf{0.925}}  & 0.919                            & {\color{mygreen} \textbf{0.930}} & 0.920                            & 0.916                           & 0.895                            & 0.924                            & {\color{reda} \textbf{0.934}}    \\
                                                       & F$^{avg}_{\beta}$ $\uparrow$    & 0.890            & 0.904             & 0.916                            & {\color{myblue} \textbf{0.925}}  & 0.916                            & {\color{mygreen} \textbf{0.927}} & 0.920                            & 0.913                           & 0.921                            & 0.923                            & {\color{reda} \textbf{0.931}}    \\
                                                       & E$^{adp}_{m}$ $\uparrow$        & 0.916            & 0.943             & 0.942                            & 0.946                            & {\color{myblue} \textbf{0.952}}  & 0.951                            & 0.949                            & 0.943                           & 0.932                            & {\color{mygreen} \textbf{0.953}} & {\color{reda} \textbf{0.957}}    \\
 \multirow{-7}{*}{\rotatebox{90}{\textbf{ECSSD}}}      & E$^{avg}_{m}$ $\uparrow$        & 0.927            & 0.936             & 0.939                            & {\color{myblue} \textbf{0.948}}  & 0.944                            & {\color{myblue} \textbf{0.948}}  & 0.947                            & 0.936                           & 0.947                            & {\color{mygreen} \textbf{0.950}} & {\color{reda} \textbf{0.953}}    \\ \hline
                                                       & S$_{m}$ $\uparrow$              & 0.907            & 0.903             & 0.916                            & 0.917                            & {\color{mygreen} \textbf{0.920}} & {\color{myblue} \textbf{0.919}}  & {\color{myblue} \textbf{0.919}}  & 0.915                           & 0.917                            & {\color{myblue} \textbf{0.919}}  & {\color{reda} \textbf{0.929}}    \\
                                                       & F$^{\omega}_{\beta}$ $\uparrow$ & 0.859            & 0.865             & 0.876                            & {\color{myblue} \textbf{0.900}}  & 0.889                            & {\color{mygreen} \textbf{0.904}} & 0.890                            & 0.880                           & 0.894                            & 0.897                            & {\color{reda} \textbf{0.917}}    \\
                                                       & MAE $\downarrow$                & 0.039            & 0.037             & 0.034                            & {\color{mygreen} \textbf{0.028}} & 0.031                            & {\color{mygreen} \textbf{0.028}} & 0.031                            & 0.033                           & 0.031                            & {\color{myblue} \textbf{0.029}}  & {\color{reda} \textbf{0.024}}    \\
                                                       & F$^{adp}_{\beta}$ $\uparrow$    & 0.871            & 0.882             & 0.896                            & {\color{myblue} \textbf{0.910}}  & 0.898                            & {\color{mygreen} \textbf{0.914}} & 0.901                            & 0.899                           & 0.899                            & 0.909                            & {\color{reda} \textbf{0.923}}    \\
                                                       & F$^{avg}_{\beta}$ $\uparrow$    & 0.878            & 0.884             & 0.894                            & {\color{myblue} \textbf{0.910}}  & 0.901                            & {\color{mygreen} \textbf{0.913}} & 0.903                            & 0.897                           & 0.904                            & 0.909                            & {\color{reda} \textbf{0.923}}    \\
                                                       & E$^{adp}_{m}$ $\uparrow$        & 0.938            & 0.945             & 0.953                            & 0.958                            & 0.956                            & {\color{mygreen} \textbf{0.960}} & 0.957                            & 0.953                           & 0.953                            & {\color{mygreen} \textbf{0.960}} & {\color{reda} \textbf{0.965}}    \\
 \multirow{-7}{*}{\rotatebox{90}{\textbf{HKU-IS}}}     & E$^{avg}_{m}$ $\uparrow$        & 0.930            & 0.935             & 0.935                            & {\color{myblue} \textbf{0.952}}  & 0.944                            & {\color{mygreen} \textbf{0.953}} & 0.948                            & 0.937                           & 0.947                            & {\color{myblue} \textbf{0.952}}  & {\color{reda} \textbf{0.960}}    \\ \hline
                                                       & S$_{m}$ $\uparrow$              & 0.845            & 0.838             & {\color{mygreen} \textbf{0.865}} & 0.857                            & {\color{myblue} \textbf{0.864}}  & 0.859                            & {\color{myblue} \textbf{0.864}}  & 0.854                           & 0.859                            & 0.854                            & {\color{reda} \textbf{0.869}}    \\
                                                       & F$^{\omega}_{\beta}$ $\uparrow$ & 0.785            & 0.789             & 0.813                            & 0.823                            & 0.819                            & {\color{mygreen} \textbf{0.829}} & {\color{myblue} \textbf{0.824}}  & 0.804                           & 0.823                            & 0.818                            & {\color{reda} \textbf{0.847}}    \\
                                                       & MAE $\downarrow$                & 0.075            & 0.079             & 0.066                            & 0.064                            & {\color{myblue} \textbf{0.063}}  & {\color{mygreen} \textbf{0.062}} & 0.066                            & 0.071                           & 0.066                            & 0.066                            & {\color{reda} \textbf{0.057}}    \\
                                                       & F$^{adp}_{\beta}$ $\uparrow$    & 0.771            & 0.815             & 0.837                            & {\color{myblue} \textbf{0.844}}  & 0.839                            & {\color{mygreen} \textbf{0.853}} & 0.842                            & 0.830                           & 0.797                            & 0.840                            & {\color{reda} \textbf{0.861}}    \\
                                                       & F$^{avg}_{\beta}$ $\uparrow$    & 0.814            & 0.819             & 0.840                            & 0.843                            & 0.840                            & {\color{mygreen} \textbf{0.851}} & {\color{myblue} \textbf{0.849}}  & 0.835                           & 0.843                            & 0.841                            & {\color{reda} \textbf{0.863}}    \\
                                                       & E$^{adp}_{m}$ $\uparrow$        & 0.847            & 0.877             & 0.886                            & 0.892                            & {\color{myblue} \textbf{0.899}}  & {\color{mygreen} \textbf{0.903}} & 0.893                            & 0.882                           & 0.866                            & 0.897                            & {\color{reda} \textbf{0.913}}    \\
 \multirow{-7}{*}{\rotatebox{90}{\textbf{PASCAL-S}}}   & E$^{avg}_{m}$ $\uparrow$        & 0.877            & 0.876             & 0.887                            & 0.895                            & 0.895                            & {\color{mygreen} \textbf{0.900}} & {\color{myblue} \textbf{0.897}}  & 0.881                           & {\color{myblue} \textbf{0.897}}  & 0.894                            & {\color{reda} \textbf{0.912}}    \\
 \bottomrule[1pt]
\end{tabular}%


==> tables/hmu.tex <==
\begin{tabular}{c|ccccc}
 \toprule[2pt]
 \rowcolor{tabtitle}
 Number of Groups & S$_{m}$ $\uparrow$ & F$^{\omega}_{\beta}$ $\uparrow$ & MAE $\downarrow$ & F$_{\beta}$ $\uparrow$ & E$_{m}$ $\uparrow$ \\ \midrule[1pt]
 4                & 0.836              & 0.723                           & 0.029            & 0.761                  & 0.905              \\ \rowcolor{ours}
 6                & 0.838              & 0.729                           & 0.029            & 0.766                  & 0.911              \\
 8                & 0.836              & 0.726                           & 0.029            & 0.763                  & 0.907              \\
 \bottomrule[2pt]
\end{tabular}%

